On The Role of Prompt Construction In Enhancing Efficacy and Efficiency of LLM-Based Tabular Data Generation

LLM-based data generation for real-world tabular data can be challenged by the lack of sufficient semantic context in feature names used to describe columns. We hypothesize that enriching prompts with domain-specific insights can improve both the quality and efficiency of data generation. To test this hypothesis, we explore three prompt construction protocols: Expert-guided, LLM-guided, and Novel-Mapping. Through empirical studies with the recently proposed GReaT framework, we find that context-enriched prompts lead to significantly improved data generation quality and training efficiency.

==> sections/related-work.tex <==
 work has been dedicated around using different architectures for the purpose of tabular data generation. These architectures include \citep{tgan}, \citep{ctgan} among others. However, these are based on Generative Adversarial Networks, whereas our work is based on \gls{llms} since \gls{llms} have been trained and fine-tuned on various different data types recently.~\citep{fatemi2023talk} encodes graphs as text for reasoning with an~\gls{llm}. Unlike their focus on reasoning with graph-encoded text, our work aims to enhance the quality of generated samples through improved prompt construction. Another work encoding tabular data as the text for \gls{llm} fine-tuning is~\great. We use this work as our baseline and compare the performance against our proposed prompt strategies with respect to the quality of the generated data.~\citep{hegselmann2023tabllm} propose a method to serialize the table rows as text sequences, while our approach centers on not only using the information provided but also augmenting them with semantic information. 
